A Computational Approach to Understanding Empathy Expressed in Text-Based Mental Health Support

Empathy is critical to successful mental health support. Empathy measurement has predominantly occurred in synchronous, face-to-face settings, and may not translate to asynchronous, text-based contexts. Because millions of people use text-based platforms for mental health support, understanding empathy in these contexts is crucial. In this work, we present a computational approach to understanding how empathy is expressed in online mental health platforms. We develop a novel unifying theoretically-grounded framework for characterizing the communication of empathy in text-based conversations. We collect and share a corpus of 10k (post, response) pairs annotated using this empathy framework with supporting evidence for annotations (rationales). We develop a multi-task RoBERTa-based bi-encoder model for identifying empathy in conversations and extracting rationales underlying its predictions. Experiments demonstrate that our approach can effectively identify empathic conversations. We further apply this model to analyze 235k mental health interactions and show that users do not self-learn empathy over time, revealing opportunities for empathy training and feedback.

==> analysis_old.tex <==
\section{Model-based Insights into Mental Health Platforms}
\label{sec:analysis}

%\ashish{emphasis on validity -- what does it mean? Why do we care?}

%\ashish{Whatever you are doing is relating to positive outcomes. We did ...., none of these groups really improve... more }
We next study the relationship of empathic conversations with online peer-to-peer support dynamics and likely conversation outcomes. We apply our approach to a carefully filtered dataset of 235k mental health related interactions on TalkLife.\footnote{The TalkLife dataset contains rich signals such as whether the seeker liked the response post. Since Reddit lacks equivalent publicly available signals we focus our analysis on TalkLife alone.} We use a seeker-reported indicator to identify conversations related to significant mental health challenges on TalkLife. This ensures that our analysis is not biased by widely prevalent social media interactions on these platforms (e.g., \textit{Merry Christmas to all}). 

\begin{figure}
\centering
% \vspace{-15pt}
\subfloat[Overall empathy score is obtained by adding the level of communication across the three mechanisms]{
	\label{subfig:likes-overall}
	\includegraphics[width=0.45\columnwidth]{images/like-analysis-combined.pdf} }
\hfill
\subfloat[Individual Communication Mechanisms]{
	\label{subfig:likes-ind}
	\includegraphics[width=0.45\columnwidth]{images/like-analysis-independent.pdf} } 

% \vspace{-5pt} 
\caption{Stronger communications of emotional reactions and interpretations are received positively by the seekers. Stronger explorations receive less positive feedback but receive greater number of replies leading to greater degrees of engagement. 
\tim{need to show the replies :)}}
\label{fig:likes}
% \vspace{-10pt}
\end{figure}


We study the correlations of empathic conversations with indicators of conversation outcomes (\cref{subsec:outcomes}), check whether empathy can help form relationship between users (\cref{subsec:alliance}), examine its relationship with gender (\cref{subsec:gender}), and analyze if peer supporters self-learn empathy with time (\cref{subsec:self-learn}). We end with a proof-of-concept study on providing actionable feedback to peer supporters for expressing more empathy in conversations (\cref{subsec:proof-of-concept}).


% This is useful in guiding empathy-based feedback and training methods for peer supporters online. 

%\tim{we haven't talked much about any feedback yet. discuss together. I think just say we apply model to super large dataset in order to study how empathy is expressed and responded to in the wild/at scale.}



%\ashish{Re-apply this model to a set of significant mental health concerns -- measure empathy where it is most needed. Seekers explicitly denote it as a mental health challenge. This is not just people replying without empathy on random posts, but carefully fitered posts of mental health challenges.}


%\ashish{We do not perform an equivalent analysis on Reddit due to missing data. TalkLife dataset has a unique benefits of x,y,Z -- point strengths}

%For all of our analysis, we apply EPITOME to our entire dataset of mental health support conversations on TalkLife for labeling them with empathy characteristics.

\subsection{Are empathic conversations important for positive outcomes in peer support?}
\label{subsec:outcomes}
%A successful conversation between seekers and peer supporters is key  . 
Positive feedback from the seeker in response to a conversation with a peer supporter is indicative of a successful interaction. Here, we operationalize positive feedback as seeker "liking" the response post and analyze whether empathic conversations are correlated with such feedback.


%the fraction of responses that receive such feedback. 
Figure~\ref{fig:likes} shows the variation of the fraction of responses that receive positive feedback with various levels of empathy. We find that stronger communications of empathy are received more positively by seekers (0.32 vs. 0.22 for overall empathy scores -- obtained by adding the level of communication across the three mechanisms -- of $\geq4$ and 0 respectively). In particular, stronger emotional reactions and interpretations receive more positive feedback (0.35 vs. 0.22; 0.33 vs. 0.24). Stronger explorations receive less positive feedback (0.15 vs. 0.27) but receive a greater number of replies () leading to greater degrees of engagement. These results suggest that our computational approach not only successfully measures empathy according to a principled framework, but that the measured empathy components may be important to online supportive conversations as indicated by the positive reactions from seekers.



%\tim{something about relationships?} \tim{always use effect sizes here in these sentences.} \tim{these results suggest that our empathy model not only successfully measures empathy according to a principled framework, but that these components of empathy may be important to online support conversations as seekers respond to them more positively.}

\begin{figure*}
\centering
% \vspace{-15pt}
\subfloat[Emotional Reactions]{
	\label{subfig:likes-ER}
	\includegraphics[width=0.65\columnwidth]{images/user-year-wise-ER-1-year.pdf} } 
\hfill
\subfloat[Interpretations]{
	\label{subfig:likes-IP}
	\includegraphics[width=0.65\columnwidth]{images/user-year-wise-IP-1-year.pdf} } 
\hfill
\subfloat[Explorations]{
	\label{subfig:likes-EX}
	\includegraphics[width=0.65\columnwidth]{images/user-year-wise-EX-1-year.pdf} } 
% \vspace{-5pt} 
\caption{Variation of empathy of users with time spent on the platform. We stratify users by the year in which they joined the platform and analyze the levels of empathy during different years in each stratum (2015, 2016, 2017, 2018). We observe that users do not increase in empathy over time indicating that users do not self-learn empathy.}
\label{fig:empathy-over-time}
\vspace{-10pt}
\end{figure*}



\subsection{Are empathic conversations related to the forming of relationships?}
\label{subsec:alliance}
Psychology research emphasizes the importance of empathy in forming alliance and relationship with seekers~\cite{watson2007facilitating}. Here, we operationalize relationship forming as seeker "following" the peer supporter after a conversation (but before the next conversation) and examine its correlation with empathic conversations. 

We find that seekers are much more likely to immediately follow peer supporters after a highly empathic conversation than after a conversation low in empathy (7.64\% vs. 4.95\% for an overall empathy score of $\geq4$ \tim{4+ might be more readable?} and 0 respectively; similar trend for all three communication mechanisms). This meaningfully reflects the social theories on empathy \tim{ref needed} and emphasizes the importance of emptahy and the effectiveness of our approach in identifying key interactions. 

%highlights the importance of .

%Note that such a "following" process is rare on TalkLife.


\subsection{Relationship to gender}
\label{subsec:gender}
Previous work has shown that seekers identifying as females are likely to receive more support in online communities~\cite{wang2018s}. Here, we ask if empathic interactions are affected by the self-reported gender of seekers and peer supporters.

We find that females are more empathic towards females (empathy levels of $\geq1$ -- 79\% of the times, $\geq4$ -- 1.6\%) than males are towards males ($\geq1$ -- 60\% , $\geq4$ -- 0.89\%), males are towards females ($\geq1$ -- 69\%, $\geq4$ -- 0.9\%), or females are towards males ($\geq1$ -- 73\%, $\geq4$ -- 1.3\%). \ashish{add social theories on empathy and gender}
\tim{I found this confusing -- perhaps only use >=1 here and make it all into a figure you can push in appendix?}

% We find that females are more empathic towards females (79\% times empathy of $\geq1$, 32\% times $\geq2$, and 1.6\% times $\geq4$) than males are towards males (60\% times empathy of $\geq1$, 26\% times $\geq2$, and 0.89\% times $\geq4$), males are towards females (69\% times $\geq1$, 28\% times $\geq2$, and 0.9\% times $\geq4$), or females are towards males (73\% times empathy of $\geq1$, 29\% times $\geq2$, and 1.3\% times $\geq4$). \ashish{add social theories on empathy and gender}


\subsection{Do peer supporters self-learn empathy with time?}
\label{subsec:self-learn}
We next investigate if the empathy of peer supporters on the platform changes with time and if they self-learn empathy. We analyze the variation of empathy of peer supporters with time spent on the platform (Figure~\ref{fig:empathy-over-time}). 

\xhdr{Potential Confounding Factors} We note that such an analysis can be affected by several confounding factors such as old vs. new users, user dropout, and low activity of several users. To account for these factors, we stratify users by the year in which they started supporting on the platform (2015, 2016, 2017) and analyze the average levels of empathy during subsequent years in each stratum. We further filter users with $\leq10$ posts and only consider users who stay on the platform for at least a year.

\xhdr{Findings and Implications} We observe that users do not increase in empathy over time (Figure~\ref{fig:empathy-over-time}). In particular, the emotional reactivity of users decreases over time () and their levels of interpretations and explorations almost remain constant (). We observe similar results across users of different groups (low activity users, highly active users, trained users). This indicates that users do not self-learn empathy and highlights the need of providing them feedback. 

\tim{good, but we don't have this much space -- maybe simplify and move stuff to appendix -- we can discuss}

\subsection{Towards actionable feedback to peer supporters}
\label{subsec:proof-of-concept}

\input{t_pilot}

We showed that we can effectively identify empathic interactions, empathy is important for successful platform dynamics, and peer supporters do not self-learn empathy. This points to critical opportunities for empathy-based feedback to peer supporters for making their interactions with seekers effective. Here, we present a small proof-of-concept study demonstrating how our approach can be used for providing actionable feedback on empathy. 

We work with three computer science students with no training in counseling and give them (seeker post, response post) pairs identified low in empathy by our approach (total empathy score $\leq1$). We show them -- (1) the levels of empathy predicted by our model, (2) extracted rationales, (3) a templated feedback \tim{reword - maybe feedback templates} explaining where the response lacks and how it can be made more empathic (based on the predicted levels, extracted rationales, definitions and examples in \ourapproach \tim{need to put this into the appendix, can say that these are examples of templates?}). We ask them to re-write the response post making use of the templated feedback. Table~\ref{tab:pilot} shows examples of re-written responses. Overall, the students were comfortable to re-write the responses with an average difficulty of 1.92 out of 5 \tim{scale is not clear - say higher more difficult...} and found the feedback useful in the re-writing process with an average usefulness rating of 3.5 out of 5. Moreover, our model indicated that the overall empathy of the interactions with the re-written responses increased from 0.833 to 3.08. \tim{this is the key -- highlight this, say how many responses this is based on} The participants, however, often found the provided examples too generic which points out opportunities to develop re-writing methods (like~\citet{yang2018unsupervised}) that can generate specific re-written prompts for empathy which
we consider a key direction for future work.
% forms our immediate future work. 


% (Refer Appendix for the used template). 

%found the feedback useful   out of 5.



%\tim{overall these sections can be compressed a bit -- it's more important to use this space to say WHAT THIS MEANS AND WHY THIS MATTERS.}


% \subsection{Improving online peer }





% gender

% SEEKER_M_M_CNT = {'0': 6532, '1': 4030, '2': 484 (4.38%)}
% SEEKER_M_F_CNT = {'0': 19432, '1': 18434, '2': 2200 (5.49%)}
% SEEKER_F_M_CNT = {'0': 8658, '1': 9653, '2': 1377 (6.99%)}
% SEEKER_F_F_CNT = {'0': 19590, '1': 30174, '2': 3958 (7.36%)}
% TOTAL_CNT = {'0': 65259, '1': 74219, '2': 9738}

% SEEKER_M_M_RATIO = {'0': 0.10009347369711458, '1': 0.05429876446731969, '2': 0.04970219757650442}
% SEEKER_M_F_RATIO = {'0': 0.29776735775908303, '1': 0.24837305811180427, '2': 0.2259190798932019}
% SEEKER_F_M_RATIO = {'0': 0.1326713556750793, '1': 0.13006103558388013, '2': 0.1414048059149723}
% SEEKER_F_F_RATIO = {'0': 0.3001884797499196, '1': 0.40655357792479013, '2': 0.4064489628260423}


% We investigate how the relatuonship of empathy with conversation outsomes, whether empathy is related to i as measured through likes, relationship , change over time -- at the start, are we measuring empathy wrong, related to positive putcomes, We ask -- One xhdr for all Results and Implications -- one figure with four subfigure. 

% We find: Figure 3(a), Figure 3(b), ... 
% Implications all together, a -- 3b, b -- replies/follows (first conv. next 24 hrs -- reflect on the entire day) -- 50% increase of the edges, c -- gender (no empathy at all (some expression of empathy -- score ), f->f, f->m, m->f, m->m), d -- over time (findings is robust to x,y,x, ... ), -- Our classification accuracy is high, our empathy predictions are correlated with like and follwo -- people are responding differently to these posts.

% This seems to be positive, people are not doing it, so feedback could help, We intentionally designed EPITOME, such that we can use the classification and feedback based on templkats (Appendix), We demonstrate the potential feedback in a simple proof-of-concept. When providing three partivipants, there empathy in responses increased from 0.8 to 3. Table 6 shows shows 2 examples that ...
